Libriheavy: a 50,000 hours ASR corpus with punctuation casing and context

In this paper, we introduce Libriheavy, a large-scale ASR corpus consisting of 50,000 hours of read English speech derived from LibriVox. To the best of our knowledge, Libriheavy is the largest freely-available corpus of speech with supervisions. Different from other open-sourced datasets that only provide normalized transcriptions, Libriheavy contains richer information such as punctuation, casing and text context, which brings more flexibility for system building. Specifically, we propose a general and efficient pipeline to locate, align and segment the audios in previously published Librilight to its corresponding texts. The same as Librilight, Libriheavy also has three training subsets small, medium, large of the sizes 500h, 5000h, 50000h respectively. We also extract the dev and test evaluation sets from the aligned audios and guarantee there is no overlapping speakers and books in training sets. Baseline systems are built on the popular CTC-Attention and transducer models. Additionally, we open-source our dataset creatation pipeline which can also be used to other audio alignment tasks.

==> json.tex <==
\begin{listing}
\footnotesize
\begin{minted}[tabsize=2]{js}
{
  "id": "01_baum_sea_fairies_64kb_0",
  "start": 243.919,
  "duration": 7.36,
  "channel": 0,
  "supervisions": [
    {
      "id": "01_baum_sea_fairies_64kb_0",
      "recording_id": "01_baum_sea_fairies_64kb",
      "start": 0,
      "duration": 7.36,
      "channel": 0,
      "language": "English",
      "speaker": "100",
      "custom": {
        "texts": [
          "The little girl was thoughtful for a moment. \"But why do folks dive in the water when the mermaids smile an' wink?\" she asked.",
          "THE LITTLE GIRL WAS THOUGHTFUL FOR A MOMENT BUT WHY DO FOLKS DIVE IN THE WATER WHEN THE MERMAIDS SMILE AND WINK SHE ASKED"
        ],
        "pre_texts": [                                                                                                                      
          "s born, and the old sailor became very fond of the baby girl. Her real name was Mayre, but when she grew big enough to walk, she took so many busy l
ittle steps every day that both her mother and Cap'n Bill nicknamed her \"Trot,\" and so she was thereafter mostly called. It was the old sailor who taught the
 child to love the sea, to love it almost as much as he and her father did, and these two, who represented the \"beginning and the end of life,\" became firm f
riends and constant companions. \"Why hasn't anybody seen a mermaid and lived?\" asked Trot again. \"'Cause mermaids is fairies, an' ain't meant to be seen by 
us mortal folk,\" replied Cap'n Bill. \"But if anyone happens to see 'em, what then, Cap'n?\" \"Then,\" he answered, slowly wagging his head, \"the mermaids gi
ve 'em a smile an' a wink, an' they dive into the water an' gets drownded.\" \"S'pose they knew how to swim, Cap'n Bill?\" \"That don't make any diff'rence, Tr
ot. The mermaids live deep down, an' the poor mortals never come up again.",
          "H A GRIFFITH FAMILY THIS WAS ABOUT THE TIME TROT WAS BORN AND THE OLD SAILOR BECAME VERY FOND OF THE BABY GIRL HER REAL NAME WAS MARY BUT WHEN SHE G
REW BIG ENOUGH TO WALK SHE TOOK SO MANY BUSY LITTLE STEPS EVERY DAY THAT BOTH HER MOTHER AND CAP'N BILL NICKNAMED HER TROT AND SO SHE WAS THEREAFTER MOSTLY CAL
LED IT WAS THE OLD SAILOR WHO TAUGHT THE GIRL TO LOVE THE SEA TO LOVE IT ALMOST AS MUCH AS HE AND HER FATHER DID AND THESE TOO WHO REPRESENTED THE BEGINNING AN
D THE END OF LIFE BECAME FIRM FRIENDS AND CONSTANT COMPANIONS WHY HASN'T ANYBODY SEEN A MERMAID AND LIVED ASKED TROT AGAIN CAUSE MERMAIDS IS FAIRIES AND AIN'T 
MEANT TO BE SEEN BY US MORTAL FOLK REPLIED CAP'N BILL BUT IF ANYONE HAPPENS TO SEE EM WHAT THEN CAP'N THEN HE ANSWERED SLOWLY WAGGING HIS HEAD THE MERMAIDS GIV
E EM A SMILE AND A WINK AND THEY DIVES INTO THE WATER AND GETS DROWNDED S'POSE THEY KNOW HOW TO SWIM CAP'N BILL THAT DON'T MAKE ANY DIFFERENCE TROT THE MERMAID
S LIVE DEEP DOWN AND THE POOR MORTALS NEVER COME UP AGAIN"
        ],
        "begin_byte": 4993,
        "end_byte": 5120
      }
    }
  ],
  "recording": {
    "id": "01_baum_sea_fairies_64kb",
    "sources": [
      {
        "type": "file",
        "channels": [
          0
        ],
        "source": "01_baum_sea_fairies_64kb.flac"
      }
    ],
    "sampling_rate": 16000,
    "num_samples": 9567080,
    "duration": 597.942,
    "channel_ids": [
      0
    ]
  },
  "custom": {
    "text_path": "Sea Fairies/text.txt"
  },
  "type": "MonoCut"
}
\end{minted}
\caption{JSON example} 
\label{json-example}
\end{listing}


\begin{listing}
\scriptsize
\begin{minted}[tabsize=2]{js}
{
  "start": 243.919,
  "duration": 7.36,
  "channel": 0,
  "supervisions": [
    {
      "language": "English",
      "speaker": "100",
      "custom": {
        "texts": [
          "... when the mermaids smile an' wink?\" she asked.",
          "... WHEN THE MERMAIDS SMILE AND WINK SHE ASKED"
        ],
        "pre_texts": [                                                                                                                      
          "... an' the poor mortals never come up again.",
          "... AND THE POOR MORTALS NEVER COME UP AGAIN"
        ],
        "begin_byte": 4993,
        "end_byte": 5120
      }
    }
  ],
  "recording": {
    "source": "01_baum_sea_fairies_64kb.flac"
    "sampling_rate": 16000,
    "duration": 597.942,
  },
  "custom": {
    "text_path": "Sea Fairies/text.txt"
  },
}
\end{minted}
\caption{The metadata for one of the segments in Libriheavy.} 
\label{metadata}
\end{listing}
